Deep Extragalactic VIsible Legacy Survey (DEVILS): Identification of AGN through SED Fitting and the Evolution of the Bolometric AGN Luminosity Function

Active galactic nuclei (AGN) are typically identified through radio, mid-infrared, or X-ray emission or through the presence of broad and/or narrow emission lines. AGN can also leave an imprint on a galaxy's spectral energy distribution (SED) through the re-processing of photons by the dusty torus. Using the SED fitting code ProSpect with an incorporated AGN component, we fit the far ultraviolet to far-infrared SEDs of $\sim$494,00 galaxies in the D10-COSMOS field and $\sim$230,000 galaxies from the GAMA survey. By combining an AGN component with a flexible star formation and metallicity implementation, we obtain estimates for the AGN luminosities, stellar masses, star formation histories, and metallicity histories for each of our galaxies. We find that ProSpect can identify AGN components in 91 per cent of galaxies pre-selected as containing AGN through narrow-emission line ratios and the presence of broad lines. Our ProSpect-derived AGN luminosities show close agreement with luminosities derived for X-ray selected AGN using both the X-ray flux and previous SED fitting results. We show that incorporating the flexibility of an AGN component when fitting the SEDs of galaxies with no AGN has no significant impact on the derived galaxy properties. However, in order to obtain accurate estimates of the stellar properties of AGN host galaxies, it is crucial to include an AGN component in the SED fitting process. We use our derived AGN luminosities to map the evolution of the AGN luminosity function for $0<z<2$ and find good agreement with previous measurements and predictions from theoretical models.

==> Intro.tex <==

\begin{itemize}
    \item AGN are SMBHs acreeting matter which in turn produces emission
    \item AGN can be visible across the entire electromagnetic spectrum from X-ray to radio and can outshine their entire host galaxy in some cases
    \item Difficulties detangling AGN emission from their hosts, and it has become apparent that the different methods of identifying AGN can select different populations sometimes with no overlap
    \item plenty of work has been done selecting AGN in X-rays, radio through jets and `excess emission', MIR colours
    \item Can also select AGN through SED fitting \cite{LejaHotDustPanchromatic2018,GuoPhysicalpropertiesCDFS2020,PouliasisobscuredAGNpopulation2020}
     \item Fitting the UV-FIR SEDs of AGN can trace the contribution from the dusty torus in the across the NIR-FIR and the contribution from the accretion disk in the very blue optical and the ultraviolet. 
    \item Observations from X-rays trace the hot corona and 'reflection' (plot from C M Harison) 
    \item Other codes exist which prioritise the AGN (AGNfitter \citealt{CalistroRiveraAGNfitterBayesianMCMC2016} and \textsc{iragnsep} \citealt{BernhardpostHerschelviewintrinsic2021}, \textsc{ARXSED}, \citealt{AzadiDisentanglingAGNstarformation2020})
    \note{all use delayed tau sfh models, with no evolving metallicity}
    and place little importance on the stellar populations
    \item With \textsc{ProSpect} we can not only model the star formation history and chemical enrichment history in a flexible manner but we can also model the AGN allowing for the extraction of accurate stellar properties simultaneously 
\end{itemize}




In seyfert galaxies, the IR emission can be roughly understood as comprising three spectral components 
\begin{enumerate}
    \item thermal radiation from dust in a compact region ambient to the active nucleus
    This component, often referred to as a "torus" can obscure direct lines of sight to the nucleus leading to distrinct observational characteristics
    \item Thermal dust continuum associated with star formation or perhaps starburst activity. This consists of line emission from macro molecules known as PAHs as well as continuum features from heated dust,
    \item additional line emission emanating from molecular, atomic and ionic species \citep{SoiferSpitzerViewExtragalactic2008}
\end{enumerate}

The dust comprising the trous is heated by the encolsed AGN central engine. This causes it to radiate in the IR bands. Its thermal spectral energy distribution thus provides an indirect measure of the AGN luminosity. This information is particularly useful for objects with heavily obscured nuclear regions for which direct measurements may not be possible. 

\cite{GallimoreColdGasActive2006}
\begin{itemize}
    \item An obscuring dusty torus should reradiate in the IR the fraction of nuclear luminosity it absorbs, and AGN continua indeed show significant IR emission. 
    \item X-ray observations reveal a large range of torus column densities, $N_H \sim 10^{22} - 10^{25} \text{cm}^{-2}$. In spite of the huge range of corresponding optical depths, the observed SEDs show only moderate variation in the infrared. 
    \item Type 2 sources display the typical $10\mu m$ dust silicate feature in absorption but the absorption depth is never large and is not well correlated with the column density inferred from X-ray observations.
    \item The $10\mu m$ feature is absent altogether in type 1 sources, even though the dust is presumably the same in both types of AGN. --> The complete absence of the $10\mu m$ feature from type 1 spectra is a consequence of the toroidal geometry of the cloud distribution.
\end{itemize}





Correlations between AGN and host galaxy properties
\begin{itemize}
    \item Local AGN (Sy 1 and Sy2) and moderate luminosity AGN in the redshift range (z = 0.4 - 1.1) tend to reside primarily in early-type (bulge dominated) galaxies
    \item AGN early-type hosts show enhanced blue global rest-frame optical colors compared to early-type inactive galaxies. This holds in low redshift (z<0.2) SDSS studies, as well as in intermediate redshifts (z $\sim$ 0.5-1.1) samples. These colors are consistent with the presence of young stellar populations, suggesting that the onset of AGN activity in intimately linked to the recent onset of global SF in the hosts.
    \item The frequency of large-scale stellar bars is significantly higher in starburst galaxies than normal galaxies. 
\end{itemize}



==> other.tex <==

From \cite{DelvecchioVLACOSMOSGHzLarge2017}
Radio selected AGN have very low accretion rates and populate overdense regions similarly to the most massive galaxies (Georgakakis + 2007, Silverman + 2009, Coil + 2009) 
In contrast, X-ray and MIR selected AGN are characterised by active star formation and less dense environments. 

Higher frequency is good for cores! - Kat Ross 

\cite{HickoxObscuredActiveGalactic2018} - The main advantage of the MIR over X-rays is that the integration times needed for AGN identification are much shorter 

X-rays are sensitive to obscured sources, especially in the harder X-ray energies, which are less affected by neutral hydrogen absorption. 


Most of the AGN found in X-ray surveys are "radio quiet" 


\cite{DelvecchioVLACOSMOSGHzLarge2017}


\subsection{Method Validation using the Brown Atlas}
%\note{I don't know how useful this section is, the BPT histograms don't look great and we've got a moderate correlation with Joel's work. I think the validation within DEVILS is more compelling evidence.}

To assess our implemented fitting method we first fit the atlas of 129 low redshift ($z<0.05$) galaxies presented in \cite{BrownAtlasGalaxySpectral2014}.
These galaxies have exquisite photometry spanning the ultraviolet to the mid-infrared and span a broad range of galaxy types.
We use imaging in the GALEX FUV and NUV bands, SDSS ugriz, 2MASS JHKs, IRAC Channels 1-4 and WISE Channels 1-4. 
This results in better wavelength coverage across the MIR regime than when fitting the DEVILS sample, but with no FIR coverage. 

\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{BPT_hist.pdf}
    \caption{Stacked histogram showing the distribution of sources from \citet{BrownAtlasGalaxySpectral2014} as a function of $f_\text{AGN}$ (upper) and AGN luminosity (lower). The colours show the classification from the BPT diagram as presented in \citet{BrownAtlasGalaxySpectral2014}, where composite objects lie between the demarcations outlined by \citet{Kauffmannhostgalaxiesactive2003} and \citet{Kewleyhostgalaxiesclassification2006}. Objects shown in black do not have a BPT classification. }
    \label{fig:BPTHist}
\end{figure}

In Table~\ref{tab:BrownAtlas} we present the obtained stellar masses, star formation rates, AGN luminosities and $f_\text{AGN}$ (measured here between $4-20\,\mu$m) from \textsc{ProSpect}. We also include the BPT classification presented in \cite{BrownAtlasGalaxySpectral2014}, and the X-ray luminosity of each object. 
Figure~\ref{fig:BPTHist} shows the distribution of AGN luminosities and $f_\text{AGN}$ coloured by the BPT class of each object. 

This sample of galaxies has also been fit using the \textsc{Prospector} SED fitting code with an AGN component as described in \cite{LejaHotDustPanchromatic2018}. 
\cite{LejaHotDustPanchromatic2018} use the CLUMPY AGN models described in details in \cite{NenkovaAGNDustyTori2008a,NenkovaAGNDustyTori2008}, which models the emission from a clumpy dust torus medium but does not include emission directly from the accretion disc which takes the form of a power law in the optical and UV.
Figure~\ref{fig:BrownFAGNComp} shows a comparison of the recovered $f_\text{AGN}$ from \textsc{ProSpect} and \textsc{Prospector} measured between $4-20\,\mu$m for consistency. 
We find strong agreement for the objects with the highest values of $f_\text{AGN}$ where the MIR is dominated by the AGN component, but find less agreement for objects with a less significant AGN contribution.
There are a number of differences between \textsc{ProSpect} and \textsc{Prospector} not limited to the differences in the AGN model that could cause this including differing star formation history parameterisations, stellar population libraries, and dust templates. 


\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{fAGN_comparisons.pdf}
    \caption{Comparison of the $f_\text{AGN}$ measured using \textsc{ProSpect} from this work for the \citet{BrownAtlasGalaxySpectral2014} sample of galaxies, and measured using \textsc{Prospector} as presented in \citet{LejaHotDustPanchromatic2018}. We show here $f_\text{AGN}$ measured between $4-20\,\mu$m for consistency with the results presented in \citet{LejaHotDustPanchromatic2018}.}
    \label{fig:BrownFAGNComp}
\end{figure}



\subsection{Radio AGN}
\begin{figure}
    \centering
    \includegraphics[width = \linewidth]{RadioExcess.png}
    \caption{Comparison between the measured flux density at 3GHz from VLA measurements and the predicted 3GHz flux density from \textsc{ProSpect} using the recovered star formation history.
    The top panel shows galaxies with $f_\text{AGN} >0.1$ and the bottom panel shows galaxies with $f_\text{AGN} < 0.1$. 
    The colour scale for both panels is the same to show the relative density of points.
    The black line denotes the one-to-one relation, the red solid line shows the running median and the dashed lines show the upper and lower quartiles. 
    }
    \label{fig:RadioExcess}
\end{figure}





AGN can be identified at radio frequencies from the existence of relativistic jets powered by a central SMBH, which are detected via the synchrotron emission of the jet \addcite. 
The objects are designated as radio-loud, and are believed to make up 10 per cent of the AGN population \addcite. 
\note{Timescales}

To compare to radio AGN, we use radio data from the VLA-COSMOS 3\,GHz Large Project \citep{SmolcicVLACOSMOSGHzLarge2017} which used 384 hours of observations with the Very Large Array (VLA) to reach an average rms sensitivity of $2.3\,\mu$Jy beam$^{-1}$ and an angular resolution of $\sim0.75''$. 
The catalogue includes 10,830 radio sources identified at peak surface brightness $\ge5\sigma$.
We position match to our catalogue with a 1'' radius using the \texttt{coordmatch} function and find radio counterparts for 6147 of our sources. We visually inspect the optical and radio source positions to ensure that we are matching the radio object to the correct optical object.

Within \textsc{ProSpect}, the SFH recovered from fitting to the FUV-FIR can be used to predict the emission of the galaxy in radio frequencies using a mixture of free-free (thermal) and synchrotron (non-thermal) radio emission using a prescription based on the work of \cite{MarvilIntegratedRadioContinuum2015}.
The predicted radio emission from \textsc{ProSpect} models only the contribution from star formation and does not include emission from AGN.
We can therefore use the predicted radio emission from \textsc{ProSpect} to compare to the measured fluxes, and can make the physical assumption that any significant excess in the observed flux is due to the contribution from an AGN component (see \citealt{DelvecchioVLACOSMOSGHzLarge2017}).

Figure~\ref{fig:RadioExcess} shows the comparison between the predicted 3\,GHz emission from \textsc{ProSpect} and the measured VLA 3\,GHz emission. 
The upper panel shows objects with a significant AGN contribution ($f_\text{AGN} > 0.1$) as measured by \textsc{ProSpect} and the bottom panel shows objects with $f_\text{AGN} < 0.1$. 
For objects with no significant AGN contribution ($f_\text{AGN} < 0.1$), we find that the majority of objects have predicted 3\,GHz fluxes that agree with the VLA measurements. 
We find that almost all objects with a significant AGN contribution ($f_\text{AGN} > 0.1$) have a larger measured flux than predicted from the stellar component alone.
This supports the idea that there is an AGN contribution to the radio flux not included in the prediction from \textsc{ProSpect}. 

We find some objects with no significant AGN contribution with larger observed fluxes than predicted. 
This might be expected as the radio jets trace longer timescales than the accretion onto the SMBH and can still be detected after an AGN has stopped acreeting.
Vice versa, we might not find excess radio emission for galaxies with a significant MIR AGN component because the jets have not yet `turned on'.




AGN can also be identified through the presence of broad and/or narrow emission lines in their optical spectra \citep[e.g.][]{SeyfertNuclearEmissionSpiral1943,BaldwinClassificationparametersemissionline1981,KewleyTheoreticalModelingStarburst2001,MeyerQuasarscompletespectroscopic2001,Kauffmannhostgalaxiesactive2003}. 
Broad lines can have typical gas velocities of a few 1000 km s$^{-1}$ and are believed to emanate from material close to the central SMBH. 
The lines are Doppler broadened because the emitting material is in gravitationally bound high velocity orbits around the SMBH.
AGN can also display narrow emission lines, with gas velocities between 300 and 1000 km s$^{-1}$, originating in the narrow line region with sizes on the order of hundreds of parsec to kiloparsec scales located above and below the plane of the dust \citep{PadovaniActivegalacticnuclei2017}.
These are often associated with forbidden atomic transitions (e.g., [O III]\,$\lambda$5007), indicative of low-density plasmas.
